Unsupervised Domain Adaptation for Self-Driving from Past Traversal Features

The rapid development of 3D object detection systems for self-driving cars has significantly improved accuracy. However, these systems struggle to generalize across diverse driving environments, which can lead to safety-critical failures in detecting traffic participants. To address this, we propose a method that utilizes unlabeled repeated traversals of multiple locations to adapt object detectors to new driving environments. By incorporating statistics computed from repeated LiDAR scans, we guide the adaptation process effectively. Our approach enhances LiDAR-based detection models using spatial quantized historical features and introduces a lightweight regression head to leverage the statistics for feature regularization. Additionally, we leverage the statistics for a novel self-training process to stabilize the training. The framework is detector model-agnostic and experiments on real-world datasets demonstrate significant improvements, achieving up to a 20-point performance gain, especially in detecting pedestrians and distant objects. Code is available at https://github.com/zhangtravis/Hist-DA.

==> sections/new_intro.tex <==
\section{Introduction}
\label{sec:intro}
Self-driving cars need to detect objects like cars and pedestrians and localize them in 3D to drive safely.
3D object detection systems have advanced rapidly in accuracy, but still fail to generalize across the extremely diverse domains where vehicles are deployed:
A perception system trained in sunny California may never have seen snow-covered cars, and may fail to detect these cars with disastrous consequences. 
Unfortunately, we cannot afford to separately annotate training data for every location a car might be driven in.
We therefore need ways of adapting 3D perception systems to new driving environment without labeled training data.
This is the problem of \emph{unsupervised domain adaptation}, where the object detector must be adapted to a new \emph{target} domain where only unlabeled data is available.




% Collecting labeled data in all corners of the world can be prohibitively expensive, but unlabeled data is much cheaper. 
% This is the setting of unsupervised domain adaptation: unlabeled training data is available in the \emph{target} domain, where good performance actually matters, in addition to labeled data in a \emph{source} domain that could potentially be quite different. For self-driving, the target domain could be a stormy corner of rural New York, while the source is sunny California.

Our application is 3D object detection from LiDAR data.
Different from prior work in unsupervised domain adaptation, we use repeated traversals of the same locations to more easily discover the invariance across domains.
For example, roads and intersections are usually visited many times by many vehicles.
Prior work has shown that the additional information from repeated traversals helps 3D detection in the same domain.
We show that this information is especially helpful for unsupervised domain adaptation.
Our setting is arguably more realistic, since data with repeated traversals are much more easily obtained without labels.

When the same location is viewed multiple times instead of only once, summarizing its similarities and differences from another location should intuitively be much easier.
To formalize this intuition, we use the repeated traversals to compute a \emph{P2 score} -- a heuristic for distinguishing between non-static versus static points \cite{}. Our hypothesis is that features that distinguish between stable vs. ephemeral objects should be invariant across domains. Yu: I didn't understand this example... pedestrians tend to walk along the sides of the road and cars -- no matter their shape -- are ephemeral and do not stay static between scenes.

Using the P2 score, we propose a simple and efficient framework for domain adaptation. Yu: I didn't edit after this. We use a neural network to featurize traversals within the same location into an efficient format similar to work by \cite{hindsight}. In the source domains (similar to a model prior to shipment), we enforce this invariance by training the featurizer to predict the P2 score along with the downstream task of 3D object detection. In the end-user domain, we additionally adapt this model by training on the \emph{locally computed} P2 score, which enforces that the model learns features pertinent to that domain. After adaptation, the locally-featurized information can be efficiently stored and queried to improve the detection in that specific domain.       

We validate our method on two large, real-world datasets: Ithaca365 \cite{} and Lyft \cite{}, as well as a suite of representative object detectors. Our method, which we term \methodlong, can achieve up to 20 points in improvement, most notably in difficult cases such as detecting pedestrians and far away objects. Furthermore, our method requires very little tuning to achieve strong performance for 3D object detection. Concretely, our contributions are as follows:

\begin{itemize}[itemsep=.3em]
    \item Potato
    \item Potato 2
    \item Moaarrr Potatoes
\end{itemize}
